Straightening Out the Straight-Through Estimator: Overcoming Optimization Challenges in Vector Quantized Networks

This work examines the challenges of training neural networks using vector quantization using straight-through estimation. We find that a primary cause of training instability is the discrepancy between the model embedding and the code-vector distribution. We identify the factors that contribute to this issue, including the codebook gradient sparsity and the asymmetric nature of the commitment loss, which leads to misaligned code-vector assignments. We propose to address this issue via affine re-parameterization of the code vectors. Additionally, we introduce an alternating optimization to reduce the gradient error introduced by the straight-through estimation. Moreover, we propose an improvement to the commitment loss to ensure better alignment between the codebook representation and the model embedding. These optimization methods improve the mathematical approximation of the straight-through estimation and, ultimately, the model performance. We demonstrate the effectiveness of our methods on several common model architectures, such as AlexNet, ResNet, and ViT, across various tasks, including image classification and generative modeling.

==> 2_related_works.tex <==
\section{Related works}

Vector-quantization~\cite{gray1984vector}~(VQ) is a competitive ``winner-takes-all'' framework that uses prototype vectors to cluster the input data. Originally used for efficient digital communication, quantization formms for the foundation of lossy compression algorithms like JPEG.
VQs are related to online K-means.
There has been renewed interests in VQ methods with its success deep generative models. \cite{van2017neural} proposed VQ-VAE, a class of generative model, that uses vector-quantization over traditional approach of variational inference~\cite{kingma2013auto}. Notable works that build upon VQ-VAE are: Taming-transformers~\cite{esser2020taming}, VQ-VAE2~\cite{razavi2019generating}, and DALL-E~\cite{ramesh2021zero}. 
Beyond generative models, \cite{ozair2021vector} explores the use of VQ for model planning.
Integrating VQs with deep nets provides a discrete and a more disentangled representation of the model, often a desirable properties for down stream task. Yet, training such models have proven to be difficult~\cite{kaiser2018fast, lancucki2020robust}.
For these reasons, training models with multiple VQ layers have shown to be very difficult.
We are not the first work to use apply multiple VQ-layers and to mention few works that do: \cite{harwath2019learning} uses 2 VQ layers for speech grounding, \cite{williams2020hierarchical} uses 2 VQ layers for image compression, \cite{razavi2019generating} uses residual connections to train 2 VQ layer for coarse-to-fine image synthesis, and~\cite{lee2022autoregressive} propose to model the residual error using 4 VQ, although not hierarchical. 
The ability to stack multiple VQ layers, to date, is still very limited. Mainly because to obtain discrete hierarchical representation comes with degradation in performance. For these reasons, VQ methods have been mostly unused in domains beyond generative models.
In this work, we aim to tackle this status-quo by systematically investigating the issues that arises in vector-quantization. We propose methods to improve the stability of hierarchical vector-quantized networks.
\pulkit{This section illustrates the successes and failures of VQ methods -- we can use this as part of the introduction.}








==> checklist.tex <==

\section*{Checklist}


The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} we use an existing dataset.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{} The error bars are negligible for classification. Omitted for clarity of the figures.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{} appendix.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
   \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old_4_method.tex <==
\section{Improving optimization of vector-quantized networks}
A naive implementation of VQN performs worse on the task it was trained to solve than its non-quantized baseline. Illustrated in~\fig{fig:vq_hurts}, adding a VQ layer for classification performs noticeably worse and,  
as a matter of fact, the hierarchical counterpart does not train.
The instabilities mainly arise from \textit{quantization error} and \textit{under-training} of the codebook. Our work investigates and addresses these issues by proposing a better VQ design and a new VQ framework called \textit{grouped vector-quantization (GVQ)} that controls the granularity of the discrete representation.
\input{./figures/distribution_histogram}

\subsection{Reducing approximation error}
\label{sec:approx}
To ensure that the correct gradient flows through the quantization layer, one must reduce the error introduced from the straight-through approximation. For ease of understanding, consider a network with a single VQ layer. Let $\mathcal{L}^*$ be the loss when the quantization step was skipped (\eg $F_2(F_1(x))$) and $\mathcal{L}$ be the loss computed in the presence of the quantization function (\eg $F_2(h(F_1(x)))$). The gradient with respect to these losses describes the gradient the encoder \textit{expected} to receive and the gradient it \textit{actually} received. The difference between these terms characterizes the gradient error of vector-quantization:
\begin{align}
\underbracket[0.140ex]{\left\lVert \frac{\partial \mathcal{L}^*}{\partial F_1} - \frac{\partial \mathcal{L}}{\partial F_1} \right\rVert}_{\mathsf{VQ\; approximation\;error}} \propto \left\lVert \frac{\partial F_2(\bz_e) }{ \partial \bz_e} - \frac{\partial F_2(\bz_q)}{ \partial \bz_q} \right\rVert 
\end{align}
The gradient approximation error is a composition of errors introduced from generating a different prediction than intended and the straight-through estimation.
One can see that the approximation error is small when (1) \textbf{the quantization error is small} and (2) \textbf{the decoder function $F_2$ is smooth}, where the decoder functions refers to the layers proceeding the quantization function.
To see this, consider the case when $\bz_e$ and $\bz_q$ are equivalent, then the estimation error is $0$. When the are not equivalent and $F_2(\cdot)$ is smooth, then the approximation error is proportionately bounded by the quantization error $d(\bz_e, \bz_q)$.
By reducing the approximation error, we hope to minimize the discrepancy between the performance of the vector-quantized model and its non-quantized counterpart. 


\subsubsection{Quantization Function}
\label{sec:quantization}
The quantization function is an important aspect for improving the stability of training. 
Careful design of the quantization function $h(\cdot, \cdot)$ and its associated codebook $\mathcal{C}$:  $\min_{\mathcal{C}} h(\bz_e, \mathcal{C})$ can reduce the approximation error and stabilize training. 


\xpar{Codebook initialization --} The goal of the quantization function is to generate $\bz_q\sim\mathcal{C}$ that closely matches that of $\bz_e\sim\mathcal{Z}_e$ -- here $\bz_q$ is sampled from codebook $\mathcal{C}$ using a discrete deterministic sampler $d$ (the distance function), and $\mathcal{Z}_e$ is a parametric distribution modeled by the network. 
Large gradient errors introduced by badly initialized codebooks are among the primary causes of training instability.
Typically the codebook vectors are initialized as samples from a fixed distribution. By minimizing the divergence between $\mathcal{C}$ and $\mathcal{Z}_e$ we can minimize the gradient errors.
Unfortunately, computing this divergence requires apriori knowledge of embedding distribution $\mathcal{Z}_e$ -- how the input distribution is featurized by each layer at initialization. 
While one could use domain knowledge of the distribution and match the moments to the embedding distribution before training (as illustrated in \fig{fig:toy_div}),
the challenge is that there is no one-size-fits-all codebook distribution across and within models. 
For example, putting the same distribution on a residual connection, a different activation function, and even at a different depth would result in a rather large divergence~(see \app{app:dist}).  

To overcome this challenge, we use data-dependent initialization, which is agnostic to the distributional assumption. 
We first compute feature embeddings for many training data points at initialization. From this set, we randomly select a subset and use them as initialization for code-vectors. Using $K-$means instead of random selection results in similar performance. In~\fig{fig:toy_div}, we compare different distributions for initializing the code-vectors against data-dependent initialization. We observed that data-dependent initialization has the smallest empirical KL-divergence between $\bz_e$ and $\bz_q$. 
Next, we study the effect of the initial divergence in downstream task performance. For this, we trained $\mathsf{ResNet18}$ with $\mathsf{3VQ}$ layers on $\mathsf{TinyImageNet}$. Figure~\ref{fig:init_comparisons} shows that the divergence of the distribution at initialization correlates with model performance.
The use of data-dependent approaches has also been explored in~\cite{lancucki2020robust} and noted in a recent code repository~\cite{dvq2021karpathygithub}. Yet a much-needed formal investigation of its importance is missing, which our work aims to fill. \cite{lancucki2020robust} uses K-mean to reinitialize the codebook during training repeatedly, and~\cite{dvq2021karpathygithub} uses data-dependent initialization.



\xpar{Bounded measure space: cosine distance --} 
In the limit of infinitely-sized codebook, where the code-vectors are generated from a distribution that span $\mathcal{Z}_e$, the quantization error is perfectly minimized: $\lim_{|\mathcal{C}| \rightarrow \infty} \min_j d(\bz_e, \bc_j) \rightarrow 0$. 
Although such a design is computationally impractical, one would expect to see that simply increasing the size of the codebook improves the model's performance. Contrary to expectation, the performance does not increase. As shown in~\fig{fig:index_collapse} the number of active codes does not increase as more codes are used even with data-dependent initialization.
This is a well-known phenomena called \textit{index-collapse}~\cite{van2017neural}. Index collapse, also known as poster collapse, occurs when the norm of the weights grows during training~\cite{}, causing a positive feedback loop where both the embedding and the code-vectors reinforce each other and increase in magnitude. While the norm of the selected code-vectors increases, other code vectors are no longer trained. 

One can overcome this issue by using a bounded measure-space for the quantization function. Here, we propose to use cosine-distance, which computes the angular distance on a unit-sphere. Cosine distance is easy to implement, has bounded error, and enjoys many of the same convergence properties as euclidean distance:
$d_\mathsf{cos}(\bx, \by) =  \frac{1}{2} d_\mathsf{euc} ( \bx / \lVert \bx \rVert,  \by / \lVert \by \rVert )^2$ .
To extend vector-quantization to cosine-distance one can either normalize $\lVert \bz_e \rVert = \lVert \bz_q \rVert = 1$ ($\mathsf{unit}$-$\mathsf{norm}$) or match the vector-norm of $\lVert \bz_q \rVert $ to that of $\lVert \bz_e \rVert$ ($\mathsf{re}$-$\mathsf{norm}$) after querying with cosine distance. We show performance of both variation in~\fig{fig:cos_ablate}. We find that cosine distance outperforms euclidean distance, is robust to hyper-parameters, and does not suffer from exploding gradients and errors. 

\input{./figures/index_extreme}
\input{./figures/smoothing}












\subsubsection{Ensuring smoothness via minimizing representation divergence.}

Ensuring that the network is smooth bounds the gradient error to be proportional to the quantization error.
Smoothness can be guaranteed by enforcing the function $f$ to be smooth. This can be described by a contractive mapping: $\lVert f(\bz_e) - f(\bz_q) \rVert \leq k \cdot \lVert \bz_e - \bz_q \rVert $, wher $k$ is the Lipschitz constant that describes the smoothness of the function $f(\cdot)$ (\eg small $k$-Lipschitz implies smooth $f(\cdot)$). 
In our case that uses a single VQ, we desire the decoder function $F_2 = f$ to be smooth.
As we have access to $\bz_e$ and $\bz_q$, we can directly regularize for the smoothness of the decoder by minimizing the distance of the feature representations $\min \lVert f(\bz_q)$ - $f(\bz_e) \rVert = \mathcal{L}_{\mathsf{smooth}}$. Where $F_2(\bz_e)$ is the prediction generated from the model with the vector-quantization layers skipped. 
When smoothing, we augment our final objective with $\mathcal{L}_{\mathsf{vq}} + \gamma \cdot \mathcal{L}_{\mathsf{smooth}}$, where we use $\gamma=1$.
We observed smoothing to stabilize training and help as more VQ layers are added. 
Smoothing, however, requires $2$ forward passes, and therefore, we found it most beneficial when using more than $3$ VQ layers on a network with more than $12$ layers. While the models we experimented with are largely insensitive to the choice of $\gamma$, we found using too large of a value to hurt performance.










\subsection{Grouped Vector Quantization}
With the methods proposed above, HVQNs can now enjoy stable training.
Unfortunately, these models are still shy of being able to match the performance of their continuous counterparts.
This performance disparity is partly due to the under-training of the codebook. In this section, we first study a scenario that isolates the issue of codebook under-training. We then propose grouped vector quantization to help mitigate this issue.


In VQ, choosing a large number of codebooks can reduce the quantization error. However, with a large codebook, some of the code-vectors might be infrequently chosen during the training process. 
Code-vectors that are not selected do not receive gradients and therefore might be under-trained. %
While using cosine distance does address this issue to a certain extent, we found this problem to persist.
To investigate the effect under-sampling of code vectors has on the model, we consider an experiment where we vary the rate at which code-vectors are sampled while keeping the number of model parameters and the codebook size fixed.
We achieve such a setup by varying the number of pooling layers. The goal is to compare the effect pooling has on a continuous model against VQ models.
For motivational purposes, we define $p_{\text{active}}$ to be the probability that some code-vector $i$ will activate (we make a simplifying assumptions that all codevectors activate in i.i.d manner).
Then for a CNN with input $\bx \in \mathbb{R}^{h \times w \times c}$ we have:
\begin{align}
p_\text{activate} = \frac{hw}{ |\mathcal{C} | \cdot 2^{n_{\text{pool}}}}
\end{align}
Where $h$ and $w$ are the image dimensions and $n_{\text{pool}}$ is the number of pooling layers preceding the quantization layer. 
Here we assume the pooling layer scales the spatial dimension in half.
Ensuring $p_{\text{activate}}$ to be high would imply that the code-vectors are trained consistently.
In~\fig{fig:pooling}, we observe that varying the number of pooling layers has a negligible effect on the performance of non-VQ models, while on the other hand, the performance of VQ models is largely impacted by the pooling operator (the final spatial dimension is $2\times2$). There are other ways to vary $p_\text{activate}$ such as varying the batch size, which we found to have a similar effect. 
It is also worth noting that VQ models are inherently a winner-takes-all algorithm. The information fidelity a VQ model can represent is strictly more limited than that of a continuous model. Hence, spatially pooling the model can further hurt the model's performance.
\input{./figures/gvq_diagram}
\input{./figures/pooling_grid}




\xpar{Grouped Vector Quantization (GVQ) --- } GVQ is a VQ layer that represents a vector not as a single code, but as a group of codes. The vectors are chunked into smaller $n_{\mathsf{group}}$ sub-vectors. With some abuse in notation, we denote the grouping operator as $\mathsf{group}(\bz_e, n_{\mathsf{group}}) \rightarrow \{ \bz_e^0, \dots, \bz_e^{n_\mathsf{group}} \}$.
The quantization function $h_{\mathsf{group}}(\cdot, \cdot)$ is applied to each sub-vector $\bz_e^{i}$ and the resulting vectors are re-concatenated using the $\mathsf{concat(\cdot)}$ operator:
\begin{align}
\bz_q = F_2 \left( \frac{1}{\sqrt{n_{\mathsf{group}}}} \cdot \mathsf{concat} \left( h_{\mathsf{group}}( \mathsf{group}(\mathbf{\bz_e}, n_{\mathsf{group}}), \mathcal{C}) \right) \right) \quad
\end{align}

Here, $\sqrt{n_{\mathsf{group}}}$ is the normalization constant. Notice that GVQ has many similarities to group-norm~\cite{wu2018group} and multi-headed attention~\cite{vaswani2017attention}. When sharing the same codebook $\mathcal{C}$, GVQ allows the activation rate of the code-vectors to scale linearly with the number of groups. 
\begin{align}
p_\text{activate} = n_{\mathsf{groups}} \cdot \frac{hw}{ | \mathcal{C} | 2^{n_{\text{pool}}}}
\end{align}
Using GVQ mitigates code-vector under-training, allows compositionality, and further reduces quantization error. 
In~\fig{fig:grid}, we demonstrate how the performance of the model changes as $n_{\mathsf{groups}}$ and $\lvert \mathcal{C} \rvert$ are varied. We observe that starting from $n_{\mathsf{groups}}=4$, GVQ can performs close to that of the baseline model. 
GVQ also introduces a property of interpolating between continuous and discrete representation. 
In the limit where $n_{\mathsf{groups}} = \mathsf{dim}(\bz_e)$ and $\lvert \mathcal{C} \rvert \rightarrow \infty$, quantization error is perfectly minimized and therefore GVQ is numerically equivalent to a continuous model.
Hence, varying the number of groups varies the level of discrete representation. Therefore, one can tune the number of groups based on the task and individually adjust them within the model (\eg less groups for higher layers).
Although the compositionality of codes in GVQ is often a desirable trait, it is interesting to understand how to merge the groups back into a single group.
While it is always possible to represent a GVQ with a single group using an exponentially large codebook, one may be interested in merging the codes using a small set of code vectors. This remains to be an open question to explore in future work. 

A training curve comparison between all the aforementioned techniques is in~\app{app:training}. The comparisons include accuracy, gradient errors, commitment loss.









